Introducing a framework to assess newly created questions with Natural Language Processing

Statistical models such as those derived from Item Response Theory (IRT) enable the assessment of students on a specific subject, which can be useful for several purposes (e.g., learning path customization, drop-out prediction). However, the questions have to be assessed as well and, although it is possible to estimate with IRT the characteristics of questions that have already been answered by several students, this technique cannot be used on newly generated questions. In this paper, we propose a framework to train and evaluate models for estimating the difficulty and discrimination of newly created Multiple Choice Questions by extracting meaningful features from the text of the question and of the possible choices. We implement one model using this framework and test it on a real-world dataset provided by CloudAcademy, showing that it outperforms previously proposed models, reducing by 6.7% the RMSE for difficulty estimation and by 10.8% the RMSE for discrimination estimation. We also present the results of an ablation study performed to support our features choice and to show the effects of different characteristics of the questions' text on difficulty and discrimination.

==> background.tex <==
\section{Theoretical Background}\label{sec:background}

\subsection{Item Response Theory}
%TODO rewrite this, it is almost the same as in the previous paper
The difficulty and discrimination considered in this paper come from a two-parameter IRT model [CITE], which is characterized by three latent traits (the ``two'' refers to the number of items' latent traits): i) a skill level $\theta$ associated to each student, ii) a difficulty level $b$, and iii) a discrimination $a$ associated to each assessment item. 
These latent traits are then used to compute the probability that student $i$ correctly answers question $j$ with the item response function:
\begin{equation}
\text{P}_{\text{CORRECT}} = \frac{1}{1 + e^{-a_j \cdot (\theta_i - b_j)}}
\end{equation}

According to the intuition, students with the same skill level have a lower probability of answering correctly questions with higher difficulty.
The discrimination $a$, on the other hand, affects the steepness of the item response function curve, and that is the reason why it can be used as a measure of how well an item can discriminate between students whose skill level is above or below a certain threshold (\ie{} the difficulty of the question).
Indeed, in case of a question with low discrimination, students with very different skill levels have similar probabilities of correctly answering the question.
Thus, the information that can be gathered from that item is very limited.

Given the correctness of the answers that a student gave to a set of calibrated assessment items $Q = {q_1, q_2, ..., q_{N_q}}$, it is possible to estimate the knowledge level $\tilde{\theta}$ of the student.
This is done by maximizing the result of the multiplication between the item response functions of the questions that were answered correctly and the inverse of the item response functions of the questions that were answered erroneously, with the following formula:
\begin{equation}
\tilde{\theta} = \max_{\theta} \left[ \prod_{q_j \in Q_{C}}\frac{1}{1 + e^{-a_j \cdot (\theta - b_j)}} \cdot \prod_{q_j \in Q_{W}} \left( 1 - \frac{1}{1 + e^{-a_j \cdot (\theta - b_j)}}\right) \right]
\end{equation}

In the equation above $Q_C$ is the set of questions correctly answered and $Q_W$ is the set of questions that were answered erroneously.

\subsection{TF-IDF}
Term Frequency-Inverse Document Frequency (TF-IDF) \cite{} is an Information Retrieval (IR) technique that can be used to obtain arrays of feature (named TF-IDF weight) from input documents coming from a corpus of documents.
Considering one of such feature arrays, the value of each weight represents how important is a word (or a set of words) to the corresponding document in that corpus.
The importance grows with the number of occurrences of the word in the document but it is limited by its frequency in the whole corpus: intuitively, words that are very frequent in all the documents of the corpus are not important to any of them. 
The formula used to compute the TF-IDF weight of word $w$ in document $d$ belonging to the corpus $C = {d_1, d_2 , ..., d_{N_d} }$ is the following:
\begin{equation}
\text{TF-IDF}(w, d, C) = \text{count}(w, d) \cdot \left( \log_e \frac{N_d + 1}{\text{count}(w,C)+1} + 1\right)
\end{equation}
where $\text{count}(w,d)$ is the number of occurrence of $w$ in document $d$, $N_d$ is the number of documents in the corpus $C$ and $\text{count}(w, C)$ is the number of documents in the corpus $C$ where $w$ appears.

%TODO this is probably not the right place for this... I should move it in the feature engineering part of the paper
% Since feature set generated by the formula above might be too large with respect to the number of training samples and lead to overfitting, some methods can be used to reduce the size of the input arrays (all these methods are used in the ablation study presented in this paper).
% In particular, it is possible to i) consider only the most frequent features (\ie{} the words that are the most frequent in the corpus), or ii) remove the corpus-specific stopwords (\ie{} the words that are very common in all the documents in the corpus), or iii) remove the words whose frequency is below a certain threshold.

